PLEX: Making the Most of the Available Data for Robotic Manipulation Pretraining

A rich representation is key to general robotic manipulation, but existing approaches to representation learning require large amounts of multimodal demonstrations. In this work we propose PLEX, a transformer-based architecture that learns from a small amount of task-agnostic visuomotor trajectories and a much larger amount of task-conditioned object manipulation videos -- a type of data available in quantity. PLEX uses visuomotor trajectories to induce a latent feature space and to learn task-agnostic manipulation routines, while diverse video-only demonstrations teach PLEX how to plan in the induced latent feature space for a wide variety of tasks. Experiments showcase PLEX's generalization on Meta-World and SOTA performance in challenging Robosuite environments. In particular, using relative positional encoding in PLEX's transformers greatly helps in low-data regimes of learning from human-collected demonstrations. The paper's accompanying code and data are available at https://microsoft.github.io/PLEX.

==> demo_tasks_fig.tex <==
\begin{wrapfigure}{R}{0.5\textwidth}
\centering
\includegraphics[width=\linewidth]{demonstration_tasks_bridge.png}
\caption{\setlength{\parindent}{12pt}
For the real robot deployment, demonstration trajectories were collected for three tasks: lift-pan, pick-and-place, push-into-the-sink. For each of them we had different types of object (e.g. sushi, pepper, sausage) and different distractors (e.g. chicken, milk bottle).
}
\label{fig:demo_tasks}
\end{wrapfigure}

==> play_data_fig.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{play_data.png}
\caption{
For the real robot deployment, to train the inverse dynamics model, some play data was collected, where no demonstration was given but free form trajectories.
}
\label{fig:play_data}
\end{figure}


